Lion: Minimizing Distributed Transactions through Adaptive Replica Provision (Extended Version)

Distributed transaction processing often involves multiple rounds of cross-node communications, and therefore tends to be slow. To improve performance, existing approaches convert distributed transactions into single-node transactions by either migrating co-accessed partitions onto the same nodes or establishing a super node housing replicas of the entire database. However, migration-based methods might cause transactions to be blocked due to waiting for data migration, while the super node can become a bottleneck. In this paper, we present Lion, a novel transaction processing protocol that utilizes partition-based replication to reduce the occurrence of distributed transactions. Lion aims to assign a node with one replica from each partition involved in a given transaction's read or write operations. To ensure such a node is available, we propose an adaptive replica provision mechanism, enhanced with an LSTM-based workload prediction algorithm, to determine the appropriate node for locating replicas of co-accessed partitions. The adaptation of replica placement is conducted preemptively and asynchronously, thereby minimizing its impact on performance. By employing this adaptive replica placement strategy, we ensure that the majority of transactions can be efficiently processed on a single node without additional overhead. Only a small fraction of transactions will need to be treated as regular distributed transactions when such a node is unavailable. Consequently, Lion effectively minimizes distributed transactions while avoiding any disruption caused by data migration or the creation of a super node. We conduct extensive experiments to compare Lion against various transaction processing protocols. The results show that Lion achieves up to 2.7x higher throughput and 76.4% better scalability against these state-of-the-art approaches.

==> relatedwork/relatedwork.tex <==
\section{Related Work}

% 提交，复制，恢复

Failure recovery methods are closely related to commit and replication protocols in large scale distributed databases. 
Such databases usually require both sharding and replication, which can bring high scalability and availability.
However, sharding and replication incur extra costs to confirm atomic commit among partitions and consistency among replicas, which are solved by a set of commit and replication protocols.
Hence, the design of our fast failure recovery method is inspired by many pieces of related work, including atomic commit, replication and other fast failure recovery methods.


\textbf{Atomic commit.}
Failures may happen at any time of the whole lifestyle of a transaction, including the execution of a commit protocol.
Some data, such as transaction decision and log, are indispensable for the system to continue processing transactions after recovering from the failure. 
It is common to integrate the commitment protocol and the distributed consensus protocol. 
The Paxos Commit protocol. proposed by Gray and Lamport~\cite{DBLP:journals/tods/GrayL06}, runs a Paxos consensus algorithms to replicate the commitment decision of 2PC among a set of coordinators. 
Google Spanner~\cite{DBLP:journals/tocs/CorbettDEFFFGGHHHKKLLMMNQRRSSTWW13} adopts an approach similar to Paxos Commit to perform transactional commitment, usually called 2PC/SMR. 
The most significant difference between Paxos Commit and 2PC/SMR is the distribution of coordinators. 
Paxos Commit choose to collocate multiple coordinators on the same physical node to reduce the overhead of network communication, while Spanner replicates among geo-distributed coordinators. 
More recently, Maiyya et al.~\cite{DBLP:journals/pvldb/MaiyyaNAA19} attempted to construct a Consensus and Commitment (C\&C) unification framework and presented an instantiation of a novel distributed atomic commit protocol Generalized-Paxos Atomic Commit (G-PAC) from this C\&C framework. 
Unlike traditional layered architecture, G-PAC organized 2PC and Paxos in a flattened way. 
As a result, G-PAC can reduce one round-trip communication by integrating the prepare phase of 2PC and decision replication among coordinators. 
In our method, log replication among coordinators is in parallel with reading and writing in partitions and need completing before the entrance of 2PC. 
In this way, about one round-trip communication can be reduced.
TAPIR~\cite{DBLP:conf/sosp/ZhangSSKP15}

\textbf{Replication.}
High availability is typically implemented through replication, such as the decision and log replication in commit protocols mentioned above.
Primary-backup replication is the most classic leader-based replication protocol.
However, Paxos and other consensus protocols like Raft are more popular solutions to coordinate the concurrent reads and writes to different replicas of data while providing consistency.
Based on these replication protocols, some systems optimize the latency and number of round-trip communication.
Lazy Replication~\cite{DBLP:journals/tocs/LadinLSG92} traded off a weaker and casual consistency for better performance and provided availability for master-slave databases.
COCO~\cite{DBLP:journals/pvldb/0010Y0M21} divided transactions into epochs and treated a whole epoch of transactions as the commit unit.
The key idea behind these epoch-based protocols is trading off consistency and latency for higher throughput.
Besides, when the failure happens, all transactions of the current epoch are likely to being aborted.
However, these replication protocols are orthogonal to our fast failure recovery method, which means that any replication protocol can be adopted in our method.

%3. Lazy Replicate异步副本同步
%和我们的工作正交


\textbf{Recovery methods.}
Recovery is an indispensable and expensive process of database systems that ensures the writes of committed transactions before any failure are reflected in the database after recovery. 
ARIES~\cite{DBLP:journals/tods/MohanHLPS92} is considered the gold standard method for recovery in traditional databases, which proposes a a fine-grained logging strategy and supports partial rollbacks of transactions to reduce the overhead of recovery. 
Compared with disk-based database systems, this fine-grained tuple-level logging strategy can be a bottleneck in main-memory database systems. 
Consequently, some lighter weight, coarse-grained command logging~\cite{DBLP:journals/pvldb/LometTZ11, DBLP:conf/icde/MalviyaWMS14} techniques are proposed. 
These two kind of log-based recovery methods face a performance trade-off between transaction processing and failure recovery. 
While fine-grained logging offers faster recovery than coarse-grained logging, the latter incurs lower overhead during normal transaction processing. 
Some common methods are adopted in optimizing the recovery method, such as log compression, using hardware support and parallel recovery. 
PACMAN~\cite{DBLP:conf/sigmod/WuGCT17} leverages a combination of static and dynamic analyses to parallelize the coarse-grained transaction-level logging. 
Shen et al.~\cite{DBLP:journals/pvldb/ShenCJLOT14} proposed a partition-based recovery method in distributed graph processing systems, distributing the recovery tasks to multiple compute nodes such that the recovery processing can be executed concurrently. 

